Poisson2Sparse: Self-Supervised Poisson Denoising From a Single Image

Image enhancement approaches often assume that the noise is signal independent, and approximate the degradation model as zero-mean additive Gaussian. However, this assumption does not hold for biomedical imaging systems where sensor-based sources of noise are proportional to signal strengths, and the noise is better represented as a Poisson process. In this work, we explore a sparsity and dictionary learning-based approach and present a novel self-supervised learning method for single-image denoising where the noise is approximated as a Poisson process, requiring no clean ground-truth data. Specifically, we approximate traditional iterative optimization algorithms for image denoising with a recurrent neural network that enforces sparsity with respect to the weights of the network. Since the sparse representations are based on the underlying image, it is able to suppress the spurious components (noise) in the image patches, thereby introducing implicit regularization for denoising tasks through the network structure. Experiments on two bio-imaging datasets demonstrate that our method outperforms the state-of-the-art approaches in terms of PSNR and SSIM. Our qualitative results demonstrate that, in addition to higher performance on standard quantitative metrics, we are able to recover much more subtle details than other compared approaches. Our code is made publicly available at https://github.com/tacalvin/Poisson2Sparse

==> figures/algo.tex <==
\begin{algorithm}[t]
\small{
\caption{Proposed Poisson2Sparse Training}
\label{alg:cap}
\SetKwComment{Comment}{/* }{ */}
\SetKwInput{KwInput}{Input\quad}                % Set the Input
\SetKwInput{KwOutput}{Output~}              % set the Output
\KwInput {$\noisyxmat$ a noisy image, \textit{N} Number of iterations}
\KwInput{$\bm{\theta}$ encoder-decoder parameters}
\KwOutput{denoised image $\bm{\widehat{X}}$}
\Comment{Sparse Representation Optimization via Forward Pass}

$\bm{\mathrm{A}}_0 \gets Encoder (\noisyxmat)$ \\
% \Comment{Initialize sparse code $\alpha$}
\For{$i$ \text{in} N \text{Steps}}
{

    $\bm{X_i} \gets Decoder(\bm{\mathrm{A}}_{i-1})$ \\
    % \Comment{Decode $\alpha$ to get image}
    % $\bm{R_i} \gets \bm{X_i}- \noisyxmat$ \\
    % \Comment{Compute the difference between the reconstructed image and the input}
    % Figure is incorrect this is the actual computation
    $\bm{\mathrm{A}}_i \gets S(\bm{\mathrm{A}}_{i-1} + Encoder(\noisyxmat- \bm{X_{i}}))$ \\
    % \Comment{Encode the residual and add it to the previous sparse code}
    % $\bm{\mathrm{A}}_i \gets S(\bm{\mathrm{A}}_i)$ \\
    % \Comment{Apply the soft threshold function}

}
$\bm{\widehat{X}} \gets Decoder(\bm{\mathrm{A}}_N)$\\

\Comment{Dictionary Learning via Back-propagation}

Compute $\mathcal{L}$ using ~\eqref{eq:full_loss} and update $\theta$ 
% \textbf{Loss(}\bm{\widehat{X}}, \noisyxmat)$ 
% \Comment{Loss function \eqref{eq:full_loss}}
}
\end{algorithm}

==> tables/0_related_work.tex <==
% TODO add Neighbor2Neighbor
\begin{table}[b]
    \begin{center}
    \caption{A brief comparison between different internal learning methods }
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc} 
    \hline
    Method & Explicit Prior & Sparse Repr. & Input\\
    \hline
    Deep Image Prior~\cite{8579082} & \xmark  & \xmark & Noise\\
    Self2Self~\cite{quan2020self2self}& \xmark   & \xmark & Dropout Mask \\
    Noise2Sparse (Ours) & \checkmark  & \checkmark &
    % Random
    Downsample \\
    \hline
    \end{tabular}
    }
    \end{center}
\end{table}

==> tables/1_parameter_performance.tex <==
\begin{table}[b]
    % \akash{add one more column for PSNR since DIP computation time is a lot faster we need to show how well your method works}
    % \akash{Do you have any results on performance with different dictionary size?}
    \begin{center}
    \caption{An overview of the number of parameters and computation time on the BSD68 dataset with $\lambda=5$}
    
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{lccc} 
    \hline
    Method & Parameters & Computation Time per Image & PSNR\\
    \hline
    Deep Image Prior~\cite{8579082} & $57.2 \times 10^4$  & 215s & 20.763 dB\\
    Self2Self~\cite{quan2020self2self}& $13.1 \times 10^5$   & 3419s & 25.628 dB \\
    Noise2Sparse (Ours) & $55.8 \times 10^4$ & 2091s & 24.146 dB\\
    \hline
    
    \end{tabular}
    }
    \end{center}
\end{table}

==> tables/2_notation_table.tex <==
\begin{table*}[ht]
    \begin{center}
    \caption{Notation}
    

    \begin{tabular}{lcr} 
    \hline
    Symbol & Definition & Dimensions\\
    \hline
    $d$ & Square Image width and height  & - \\
    % $W, H$ & Image width and height  & - \\
    $\bm{x},\noisyx$  &Vectorized Image& $\mathcal{R}^{d^2}$\\
    $\bm{X},\noisyxmat, \estimatexmat$ &Matrix Image& $\mathcal{R}^{d \times d}$\\
    $k$ & Dictionary Elements & - \\
    $\mathcal{D}$ & Sparse Dictionary & $\mathcal{R}^{d^2 \times k}$ \\
    $\alpha$ & Sparse Representation & $\mathcal{R}^{k \times 1}$ \\
    $m$ & Filter Size & - \\
    $D$ & Convolutional Dictionary & $\mathcal{R}^{m \times m}$ \\
    $Z$ & Sparse Feature Map & $\mathcal{R}^{d \times d}$ \\
    $\theta$ & Network Parameters & -\\
    $\mathcal{P}$ & Poisson Process &-\\
    $\lambda$ & Maximum Event Count & -\\
    $\lambda_1$ & Sparsity Regularizer Strength & -\\
    $\lambda_N$ & Neighbor2Neighbor Regularizer Strength \cite{Huang_2021_CVPR} & -\\
    $g_1, g_2$ & Random Neighbor Sampling Function &-\\
    \end{tabular}

    \end{center}
\end{table*}

==> tables/3_experiment_results_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\centering
\begin{tabular}{c|c|cccc|cccc}
\hline
 & & \multicolumn{1}{c|}{DIP}    & \multicolumn{1}{c|}{Self2Self} & \multicolumn{1}{c|}{BM3D}   & Ours            & \multicolumn{1}{c|}{DIP}           & \multicolumn{1}{c|}{Self2Self} & \multicolumn{1}{c|}{BM3D}          & Ours          \\ \hline
Dataset                                              & $\lambda$ & \multicolumn{4}{c|}{PSNR}                                                                                    & \multicolumn{4}{c}{SSIM}                                       \\ \hline
\multicolumn{1}{c|}{\multirow{3}{*}{PINCAT}} & 40        & \multicolumn{1}{c|}{30.222} & \multicolumn{1}{c|}{33.138}    & \multicolumn{1}{c|}{32.553} & \textbf{34.309} & \multicolumn{1}{c|}{.878}          & \multicolumn{1}{c|}{.942}      & \multicolumn{1}{c|}{.944} & \textbf{.957}          \\
\multicolumn{1}{c|}{}                                & 20        & \multicolumn{1}{c|}{26.495} & \multicolumn{1}{c|}{30.067}    & \multicolumn{1}{c|}{31.448} & \textbf{32.202}  & \multicolumn{1}{c|}{.765}          & \multicolumn{1}{c|}{.893}      & \multicolumn{1}{c|}{.911}          & \textbf{.937} \\
\multicolumn{1}{c|}{}                                & 10        & \multicolumn{1}{c|}{22.495} & \multicolumn{1}{c|}{27.028}    & \multicolumn{1}{c|}{27.961} & \textbf{30.005}   & \multicolumn{1}{c|}{.601}          & \multicolumn{1}{c|}{.814}      & \multicolumn{1}{c|}{.867}          & \textbf{.898} \\ \hline
FMD                                                  & -         & \multicolumn{1}{c|}{32.417} & \multicolumn{1}{c|}{28.563}    & \multicolumn{1}{c|}{29.627} & \textbf{32.980}   & \multicolumn{1}{c|}{\textbf{.916}} & \multicolumn{1}{c|}{.688}      & \multicolumn{1}{c|}{.854}          & .897        \\ \hline
\end{tabular}
% \vspace*{0.5\baselineskip}
\caption{We compare our results to both self-supervised methods such as DIP as well as traditional methods such as BM3D. The best results are in bold.}
\label{table:experiment_results}
%\vspace*{-\baselineskip}
\end{table}
